MTAG: Modal-Temporal Attention Graph for Unaligned Human Multimodal Language Sequences

Human communication is multimodal in nature; it is through multiple modalities such as language, voice, and facial expressions, that opinions and emotions are expressed. Data in this domain exhibits complex multi-relational and temporal interactions. Learning from this data is a fundamentally challenging research problem. In this paper, we propose Modal-Temporal Attention Graph (MTAG). MTAG is an interpretable graph-based neural model that provides a suitable framework for analyzing multimodal sequential data. We first introduce a procedure to convert unaligned multimodal sequence data into a graph with heterogeneous nodes and edges that captures the rich interactions across modalities and through time. Then, a novel graph fusion operation, called MTAG fusion, along with a dynamic pruning and read-out technique, is designed to efficiently process this modal-temporal graph and capture various interactions. By learning to focus only on the important interactions within the graph, MTAG achieves state-of-the-art performance on multimodal sentiment analysis and emotion recognition benchmarks, while utilizing significantly fewer model parameters.

==> figs/tex/flow.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figs/pdf/flow.pdf}
    \caption{MTGAT operation.}
    \label{fig:flow}
\end{figure*}

==> figs/tex/mult_vs_mtgat.tex <==
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{figs/img/mult_vs_mtgat.png}
    \caption{MulT vs. \CoolName. \jed{ Should we mention these differences in the method section? How to do it in a succinct way?}}
    \label{fig:mult_vs_mtgat}
\end{figure*}

==> figs/tex/teaser.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/pdf/teaser.pdf}
    \caption{Comparison between our work and previous methods.
    % which use hard alignments and employ pairwise cross-modal attention that only considers two modalities at a time.
    Our work both alleviates the need for manual alignment and considers interactions among any number of modalities at once.}
    \label{fig:teaser}
\end{figure}

==> figs/tex/unimodal.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/pdf/unimodal-align.pdf}
    \caption{Unimodal past, present, and future edge definition}
    \label{fig:unimodal_ppf}
\end{figure}

==> sections/impact.tex <==
\paragraph{Ethics Statement}
Building novel algorithms for neural modeling of multimodal language is critical to the success of AI in communication. AI systems needs to understand not just the words but also the subtle nuances of nonverbal communication. Models that are parameter efficient yet as accurate as state of the art, open the door to deployment of accurate deep models to systems with lower computational power. Subsequently, these accurate models of communication can be deployed to cell-phones and embedded systems to assist in building smart technologies; including smart healthcare applications that can better understand emotions and intention, or smart educational platforms that can understand and potentially interpret the students behavioral changes. Therefore, in terms of impact, accurate and efficient models of multimodal language are essential in the future applications of AI. 
